Compact Representations of Geometric Bipartite Graphs via Weighted Biclique Covers

Bipartite graphs are a fundamental representation for relational data arising in recommendation systems, social networks, and communication graphs. A key challenge in these settings is to store and transmit large bipartite graphs compactly while preserving exact structural and path information. We study biclique-based representations of bipartite graphs $\boldsymbol{G}=(\boldsymbol{V},\boldsymbol{U},\boldsymbol{E})$, where the edge set is encoded using a collection of complete bipartite subgraphs. We focus on the Weighted Biclique Covering problem, which minimizes the total number of vertices used across all bicliques, and introduce a generalized variant that additionally penalizes the number of bicliques, capturing practical overheads in storage, transmission, and model complexity. While the weighted biclique covering problem is known to be $\mathsf{NP}$-Complete, we show that the generalized variant is also $\mathsf{NP}$-Complete. Despite this hardness, many real-world bipartite graphs admit low-dimensional geometric embeddings or can be well approximated by them. Leveraging this observation, we develop the first approximation algorithms with provable guarantees for the (generalized) weighted biclique covering problem on geometric bipartite graphs. Specifically, for $\delta$-disk bipartite graphs in low-dimensional $\ell_\infty^d$ spaces, we design a polynomial-time algorithm that achieves an $O(\log |\boldsymbol{U}| \cdot \log^d |\boldsymbol{V}|)$-approximation, combining ideas from greedy set cover, geometric range searching, and densest subgraph optimization. We also show how our algorithms extend to $\ell_\alpha^d$ metrics for any $\alpha\geq 1$. Finally, we evaluate our algorithms on real-world bipartite datasets and show that they efficiently compute significantly smaller biclique-based representations than natural baselines, while scaling to large graphs.

==> abstractToSubmit.tex <==
The minimum biclique cover problem, also known as the bipartite dimension problem, seeks the smallest number of bicliques (complete bipartite subgraphs) needed to cover all edges of a bipartite graph $\boldsymbol{G}$. The decision version of this problem is known to be NP-complete. We investigate the complexity of two variants. The Weighted Biclique Cover problem ($\mathsf{WBC}$), first introduced by Tarjan in 1975, asks for a biclique cover that minimizes the total number of vertices used across all bicliques. The decision version of this problem is also shown to be NP-complete in unrelated domains via different proofs, highlighting its natural occurrence in various settings.
    We further introduce the Generalized Weighted Biclique Cover problem ($\mathsf{GWBC}$), which combines the objectives of the unweighted and weighted versions. Given a bipartite graph $\boldsymbol{G}(\boldsymbol{V},\boldsymbol{U},\boldsymbol{E})$ and an integer parameter $c$, the goal is to find a collection of bicliques $\mathcal{S}=\{S_1,\ldots, S_r\}$ such that $\bigcup_{S_i\in\mathcal{S}}\mathcal{E}(S_i)=\boldsymbol{E}$  and the cost $c\cdot r+\sum_{S_i\in\mathcal{S}}|\mathcal{D}(S_i)|$ is minimized, where $\mathcal{E}(S_i)$ and $\mathcal{D}(S_i)$ denote the set of edges and the set of nodes of the biclique $S_i$, respectively. In this paper, we present a new proof of NP-completeness for the $\mathsf{WBC}$ decision problem and extend the argument to show the NP-completeness of $\mathsf{GWBC}$, for any fixed integer parameter $c \geq 0$. Finally, we discuss applications of this problem and present approximation algorithms in geometric settings. In particular, for $\delta$-disk bipartite graphs in $\ell^d_\infty$ metric where $d=O(1)$, we design an $O(\log(\max\{|\boldsymbol{V}|,|\boldsymbol{U}|\})\cdot\log^{d}(\min\{|\boldsymbol{V}|,|\boldsymbol{U}|\}))$-approximation algorithm for the $\mathsf{GWBC}$ (and $\mathsf{WBC}$) problem for any parameter $c\geq 0$ that runs in polynomial time with respect to $|\boldsymbol{V}|$, $|\boldsymbol{U}|$, and $|\boldsymbol{E}|$.
    This is the first approximation algorithm for the $\mathsf{WBC}$ and $\mathsf{GWBC}$ problems in a non-trivial class of graphs.

==> experiments.tex <==
\section{Experiments}
\label{sec:exp}






\subsection{Experiment Plan}


We compare our approach against two greedy baselines that utilize different candidate generation strategies:
\begin{itemize}
    \item \textbf{RoleMiner}~\cite{10.1145/1180405.1180424}: This baseline identifies initial bicliques by grouping vertices in $V$ that possess identical neighborhoods in $U$. It iteratively merges these groups based on their intersections in $U$ to form candidates. We will refer this baseline as baseline 1.
    \item \textbf{AMBEA}~\cite{10633882}: This method employs an aggressive set-enumeration tree to exhaustively identify maximal bicliques. It utilizes an Aggressive Merge-based Pruning (AMP) technique to consolidate vertices with identical local neighborhoods, reducing the search space while maintaining maximality. We will refer this baseline as baseline 2.
\end{itemize}
Following candidate generation, both baselines employ the same greedy selection criteria as our proposed algorithm to ensure a consistent comparison.
\subsection{Experiment setting}
\subsubsection{Setup:}
All experiments were conducted on a Windows 11 workstation equipped with an Intel Core i7-9700 CPU and 32GB DDR4 RAM. Algorithms were implemented in Python 3.12.9. However, the AMBEA\footnote{https://github.com/ISCS-ZJU/AMBEA} baseline, being written in C++, was compiled as a standalone executable and invoked via subprocesses in Python. Memory performance is recorded using the Python library \textbf{psrecord}, with a 3-second pooling interval to minimize overhead.
\subsubsection{Dataset:}
We evaluate our algorithms on the following four datasets:
\begin{itemize}
    \item The \textbf{Adults} dataset~\cite{adult_2} contains around 32K records of individuals with their educations and incomes.
    \item The \textbf{Default of Credit Card Clients} dataset~\cite{default_of_credit_card_clients_350} contains 30K records of individuals with their historical credit payment data.
    \item The \textbf{MAGIC Gamma Telescope} dataset~\cite{magic_gamma_telescope_159} contains about 19K records on information and settings of high-energy particles captured by the MAGIC telescope.
    \item The \textbf{POPSIM\_1M} dataset~\cite{nguyen2023popsimindividuallevelpopulationsimulator} contains 1 million semi-synthetic records representing individual-level data with demographic information in Illinois. Only the top 2 most frequent races are selected for our experiment.
\end{itemize}
We show all statistics of our datasets for different $\delta$ values in Table~\ref{tab:datasets}.
\begin{table}[t]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Dataset & $\delta$ & $m$ & $n$ & $d$ & Grouping Attribute \\
\hline
\multirow{5}{*}{Adults} & $0.05$ & $64,280$ & \multirow{5}{*}{\num{14846}} & \multirow{5}{*}{5} & \multirow{5}{*}{Sex} \\ \cline{2-3}
                     & $0.1$ & \num{854381} &                     &                    & \\ \cline{2-3}
                     & $0.15$ & \num{2589297} &                     &                  &   \\ \cline{2-3}
                     & $0.2$ & \num{5990399} &                     &                   &  \\ \cline{2-3}
                     & $0.25$ & \num{8714044} &                     &                  &   \\ \hline
\multirow{5}{*}{Credit} & $0.002$ & \num{1538057} & \multirow{5}{*}{\num{28726}} & \multirow{5}{*}{6} & \multirow{5}{*}{Sex} \\ \cline{2-3}
                     & $0.003$ & \num{2912661} &                     &                 &    \\ \cline{2-3}
                     & $0.004$ & \num{4437255} &                     &                 &    \\ \cline{2-3}
                     & $0.005$ & \num{6034989} &                     &                 &    \\ \cline{2-3}
                     & $0.006$ & \num{7805033} &                     &                 &    \\ \hline
\multirow{5}{*}{Gamma} & $0.13$ & \num{1511959} & \multirow{5}{*}{\num{18905}} & \multirow{5}{*}{10} & \multirow{5}{*}{Class} \\ \cline{2-3}
                     & $0.14$ & \num{1961614} &                     &                 &    \\ \cline{2-3}
                     & $0.15$ & \num{2477054} &                     &                 &    \\ \cline{2-3}
                     & $0.16$ & \num{3057096} &                     &                 &    \\ \cline{2-3}
                     & $0.17$ & \num{3702052} &                     &                 &    \\ \hline
\multirow{5}{*}{POPSIM} & $0.04$ & \num{1753508} & \multirow{5}{*}{8,591} & \multirow{5}{*}{2} & \multirow{5}{*}{Race} \\ \cline{2-3}
                     & $0.06$ & \num{3090592} &                     &                 &    \\ \cline{2-3}
                     & $0.08$ & \num{4328986} &                     &                 &    \\ \cline{2-3}
                     & $0.1$ & \num{5442100} &                     &                  &   \\ \cline{2-3}
                     & $0.12$ & \num{6449440} &                     &                 &    \\ \hline
\end{tabular}
\caption{\label{tab:datasetsellinfty}Statistics of the $\delta$-disk graphs used in our experiments for $\ell_\infty^d$.}
\end{table}


\begin{table}[t]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Dataset & $\delta$ & $m$ & $n$ & $d$ & Grouping Attribute \\
\hline
\multirow{5}{*}{Adults} & $0.05$ & \num{47963} & \multirow{5}{*}{\num{14846}} & \multirow{5}{*}{5} & \multirow{5}{*}{Sex} \\ \cline{2-3}
                     & $0.1$ & \num{445724} &                     &                    & \\ \cline{2-3}
                     & $0.15$ & \num{1415555} &                     &                  &   \\ \cline{2-3}
                     & $0.2$ & \num{3016343} &                     &                   &  \\ \cline{2-3}
                     & $0.25$ & \num{5498540} &                     &                  &   \\ \hline
\multirow{5}{*}{Credit} & $0.002$ & \num{889671} & \multirow{5}{*}{\num{28726}} & \multirow{5}{*}{6} & \multirow{5}{*}{Sex} \\ \cline{2-3}
                     & $0.003$ & \num{1739709} &                     &                 &    \\ \cline{2-3}
                     & $0.004$ & \num{2710136} &                     &                 &    \\ \cline{2-3}
                     & $0.005$ & \num{3750745} &                     &                 &    \\ \cline{2-3}
                     & $0.006$ & \num{4824359} &                     &                 &    \\ \hline
\multirow{5}{*}{Gamma} & $0.13$ & \num{194737} & \multirow{5}{*}{\num{18905}} & \multirow{5}{*}{10} & \multirow{5}{*}{Class} \\ \cline{2-3}
                     & $0.14$ & \num{284626} &                     &                 &    \\ \cline{2-3}
                     & $0.15$ & \num{399339} &                     &                 &    \\ \cline{2-3}
                     & $0.16$ & \num{541050} &                     &                 &    \\ \cline{2-3}
                     & $0.17$ & \num{711158} &                     &                 &    \\ \hline
\multirow{5}{*}{POPSIM} & $0.04$ & \num{1468984} & \multirow{5}{*}{8,591} & \multirow{5}{*}{2} & \multirow{5}{*}{Race} \\ \cline{2-3}
                     & $0.06$ & \num{2660732} &                     &                 &    \\ \cline{2-3}
                     & $0.08$ & \num{3801451} &                     &                 &    \\ \cline{2-3}
                     & $0.1$ & \num{4857704} &                     &                  &   \\ \cline{2-3}
                     & $0.12$ & \num{5844122} &                     &                 &    \\ \hline
\end{tabular}
\caption{\label{tab:datasetsell2}Statistics of the $\delta$-disk graphs used in our experiments for $\ell_2^d$.}
\end{table}


\subsubsection{Preprocessing and parameter:}
Before running experiments, features were normalized for the ease of choosing value for $\delta$. In addition, duplicates were filtered before partitioning into sets $V$ and $U$ based on the grouping attributes defined above. To handle large-scale edge construction (which can reach hundreds of millions of pairs), we utilized Scipy's \texttt{KDTree} for efficient ball queries. To accommodate memory constraints, we tuned the distance threshold $\delta$ such that the number of edges is at most around 10 millions. Specific $\delta$ values and number of edges are detailed in Table~\ref{tab:datasets}. In addition, for the GWBC setting, we choose the value of c to be values in the set $\{100, 200, \dots, 500\}$
\subsubsection{Implementation}
While our theoretical framework is based on range trees, our practical implementation utilizes R-trees \cite{Guttman1984} for enhanced memory efficiency. During construction, each node $x$ precomputes and stores the vertex sets $V_x$ and $U_x$, along with the initial densest subgraph and its corresponding density. To optimize the greedy selection phase, we implement a lazy greedy strategy using a min-priority queue for each node $x$. Nodes are iteratively extracted from the heap until all edges are covered; a node's densest subgraph is included in the solution if and only if its density is unaffected by previously selected subgraphs. Regardless of inclusion, the node's densest subgraph and its density is updated before reinsertion into the heap. For the case of WBC, we use Charikar's 2-approximation~\cite{charikar2000greedy} for faster running time, and surprisingly, giving roughly the same result as the exact algorithm.\\
To integrate AMBEA's executable into Python, edges are serialized into an intermediate text file, which serves as the primary input for the executable. Following minor modifications to the original source code of AMBEA, the executable outputs the maximal bicliques to a structured text file for subsequent ingestion and processing by Python.\\
Notably, the baselines generate hundreds to thousands of times more candidates than our method, often exceeding memory limits. For example, for the WBC setting of \textbf{Adults} dataset in $\ell_\infty^d$ with $\delta=0.1$, baseline 1 provides a much better result of \num{272658} compared to \num{398443} of ours. However, baseline 1 runs in \num{5473} seconds and generates \num{1130246} candidates with peak memory usage of \num{42068} MB, far beyond our algorithm's execution time of \num{163} seconds with \num{12495} nodes/candidates and peak memory usage of \num{4208} MB. Thus, to ensure a fair and feasible comparison, we implement an early-stopping criterion. Baselines are allocated a maximum of $10-35\%$ of our algorithm's execution time, after which the generated candidate pool is finalized and greedily selected. Additionally, the consecutively generated candidates by both of our baselines tend to share many vertices. Thus, to ensure the quality of candidates, we also randomly shuffle the vertex order before generating them.
\subsection{Experimental results} \label{exp:results}
Figure~\ref{fig:wbclinf}, Figure~\ref{fig:wbcl2}, and ... demonstrates the experimental result for the three cases we mentioned.\\
First, we examine the performance for the WBC setting in $\ell_\infty^d$ and $\ell_2^d$. Overall, our algorithm shows superiority over the two baseline algorithms regarding both the number of vertices and memory despite running in less time. The gap widens progressively as we increase the values of $\delta$, with some deviations due to the random shuffle of candidates of the baselines that sometimes produce better candidates. The dominating performance can be clearly seen in the POPSIM dataset. Due to the low dimensionality and small $\delta$ values, nodes in R-Tree capture near-optimal bicliques, and thus, displaying a flat line in the result, while the our memory usage remains below the baselines'. For the Adults and Credits dataset, our algorithm provides at most 3-4 times better results compared to the baseline. Last but not least, our algorithm dominates in Gamma dataset with respect to memory, while our result scales less than that of the baselines.\\
Next, we examine the GWBC setting ... TODO.\\
Interestingly, despite not being explicitly displayed, when we experiment on extreme case where $\delta$ values that are close to 0 or 1, the baselines outperform our algorithm. Indeed, when $\delta$ is close to 0, the number of edges reduces while bicliques are less dense. Thus, the baselines tend to be able to generate every possible candidates in short amount of time and outperforms our algorithm. When $\delta$ is close to 1, the graph has tremendous amount of edges, leading to larger and denser bicliques. The baselines, even under our restriction, exploit these properties to generate large candidates that cover almost every edge, leading to good result. However, since our algorithm uses candidates generated from nodes of R-Tree where nodes are split on the median, we tend to not have access to these large candidates, leading to subpar performance.
\begin{figure*}[t]
    \centering
    \begin{tabular}{cccc}
        Adults & Credits & Gamma & POPSIM\\
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Adults_Linf_result.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Credits_Linf_result.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Gamma_Linf_result.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/POPSIM_Linf_result.pdf} \\
        \multicolumn{4}{c}{(a) Number of vertices returned by algorithms}\\[1em]
        
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Adults_Linf_memory.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Credits_Linf_memory.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Gamma_Linf_memory.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/POPSIM_Linf_memory.pdf} \\
        \multicolumn{4}{c}{(b) Peak memory used by algorithms}\\[1em]
        
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Adults_Linf_time.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Credits_Linf_time.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Gamma_Linf_time.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/POPSIM_Linf_time.pdf} \\
        \multicolumn{4}{c}{(a) Running time of algorithms}\\[1em]
    \end{tabular}

    \caption{Experimental results for WBC in $\ell_\infty^d$ across 4 datasets}
    \label{fig:wbclinf}
\end{figure*}

\begin{figure*}[t]
    \centering
    \begin{tabular}{cccc}
        Adults & Credits & Gamma & POPSIM\\
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Adults_L2_result.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Credits_L2_result.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Gamma_L2_result.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/POPSIM_L2_result.pdf} \\
        \multicolumn{4}{c}{(a) Number of vertices returned by algorithms}\\[1em]
        
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Adults_L2_memory.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Credits_L2_memory.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Gamma_L2_memory.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/POPSIM_L2_memory.pdf} \\
        \multicolumn{4}{c}{(b) Peak memory used by algorithms}\\[1em]
        
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Adults_L2_time.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Credits_L2_time.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/Gamma_L2_time.pdf} & 
        \includegraphics[width=0.22\textwidth]{figures/separate_figures/POPSIM_L2_time.pdf} \\
        \multicolumn{4}{c}{(a) Running time of algorithms}\\[1em]
    \end{tabular}

    \caption{Experimental results for WBC in $\ell_2^d$ across 4 datasets}
    \label{fig:wbcl2}
\end{figure*}
\label{sec:exp}

==> figs/arrangement.tex <==
\begin{figure}[ht]
\begin{minipage}{0.49\textwidth}
    \centering
    \begin{tikzpicture}[scale=0.25]
    \draw[thick] (0,0) rectangle (10,10);
    %\node[left] at (-0.1,8) {$\square$};
    \draw[very thick,blue] (-0.5,-2.5) rectangle (6,4);
    \draw[very thick,blue] (4.5,-0.5) rectangle (7,2);
     \draw[very thick,blue] (5,7) rectangle (10.5,12.5);
     
      \draw[red, dashed,  thick] (4.9,4.1) -- (4.9,9.9);
      \draw[red, dashed, thick] (0.1,4.1) -- (0.1,9.9);
      \draw[red, dashed, thick] (0.1,4.1) -- (9.9,4.1);
      \draw[red, dashed, thick] (0.1,9.9) -- (4.9,9.9);
      \draw[red, dashed, thick] (0.1,6.9) -- (9.9,6.9);
      \draw[red, dashed, thick] (7.1,0.1) -- (7.1,6.9);
      \draw[red, dashed, thick] (7.1,0.1) -- (9.9,0.1);
       \draw[red, dashed, thick] (6.1,2.1) -- (9.9,2.1);
       \draw[red, dashed, thick] (9.9,6.9) -- (9.9,0.1);
       \draw[red, dashed, thick] (6.1,2.1) -- (6.1,6.9);

    \node[right] at (3.2,11) {{\color{blue}$G$}};
      % Draw the middle point
    %\fill[red] (0.2,0.2) circle (1pt);
\end{tikzpicture}
\caption{The black square is a cell $\square\in\bar{V}_i$. The blue squares define the set of cells in $G_\square$ (cells already processed by our algorithm) that intersect $\square$. The red dashed segments show the arrangement of the complement of $G_{\square}$ in $\square$, i.e., the red dashed segments show $\square\cap \textsf{Arr}'(G_\square)$.}
\label{fig:arrangement}
    \end{minipage}\hfill
    \begin{minipage}{0.49\textwidth}
        \centering
        \begin{tikzpicture}[scale=0.25]
    \draw[thick] (0,0) rectangle (10,10);
    \draw[very thick,blue] (-0.5,-2.5) rectangle (6,4);
    \draw[very thick,blue] (4.5,-0.5) rectangle (7,2);
     \draw[very thick,blue] (5,7) rectangle (10.5,12.5);
     
     
    
      % Draw the middle point
    \fill[blue] (1,3) circle (4pt);
    \fill[blue] (2.5,3.7) circle (4pt);
    \fill[blue] (4.8,1.2) circle (4pt);
    \fill[blue] (6.2,8.5) circle (4pt);

     \fill[black] (0.5,7.5) circle (4pt);
     \fill[black] (1.3,9) circle (4pt);
     \fill[black] (3.1,5.2) circle (4pt);
     \fill[black] (3.8,8.2) circle (4pt);
     \fill[black] (6.5,5.8) circle (4pt);
     \fill[black] (8,2.2) circle (4pt);
     \fill[black] (9,6.5) circle (4pt);
     \fill[black] (7,6) circle (4pt);
     \node[right] at (3.2,11) {{\color{blue}$B$}};
\end{tikzpicture}
\caption{The black square is a cell $\square\in\bar{V}_i$. The blue squares define the set of heavy cells in $B_\square$ that intersect $\square$. The points represent the set of samples $H_{\square}$. Blue points are the samples in $B_\square$ while black points are the samples in $\square\setminus B_\square$. Hence, $g_\square=8$ and $M=|H_\square|=12$. If $\tau=0.3$ then $g_\square/M\geq 2\cdot \tau$, and a black point is selected as $s_\square$ with weight $\frac{8}{12}\cdot\frac{n_\square}{1-\eps'}$.}
\label{fig:sample}
    \end{minipage}
    %\caption{Combined caption for both figures}
\end{figure}


\begin{comment}
\begin{figure*}[h]
\begin{tikzpicture}[scale=0.3]
    \draw[thick] (0,0) rectangle (10,10);
    \draw[very thick,blue] (-0.5,-2.5) rectangle (6,4);
    \draw[very thick,blue] (4.5,-0.5) rectangle (7,2);
     \draw[very thick,blue] (5,7) rectangle (10.5,12.5);
     
      \draw[red, dashed,  thick] (4.9,4.1) -- (4.9,9.9);
      \draw[red, dashed, thick] (0.1,4.1) -- (0.1,9.9);
      \draw[red, dashed, thick] (0.1,4.1) -- (9.9,4.1);
      \draw[red, dashed, thick] (0.1,9.9) -- (4.9,9.9);
      \draw[red, dashed, thick] (0.1,6.9) -- (9.9,6.9);
      \draw[red, dashed, thick] (7.1,0.1) -- (7.1,6.9);
      \draw[red, dashed, thick] (7.1,0.1) -- (9.9,0.1);
       \draw[red, dashed, thick] (6.1,2.1) -- (9.9,2.1);
       \draw[red, dashed, thick] (9.9,6.9) -- (9.9,0.1);
       \draw[red, dashed, thick] (6.1,2.1) -- (6.1,6.9);

    \node[right] at (3.5,11) {{\color{blue}$G$}};
      % Draw the middle point
    %\fill[red] (0.2,0.2) circle (1pt);
\end{tikzpicture}
\caption{}
\label{fig:arrangement}
\end{figure*}
\end{comment}

==> figs/grid.tex <==
\begin{figure}[ht]
    \centering
    \begin{minipage}{0.49\textwidth}
        \centering
        \begin{tikzpicture}[scale=1.5]
    % Draw the grid
    \draw[step=0.1cm,black, thick] (0,0) grid (0.4,0.4);

    \draw[step=0.2cm,black,thick] (-0.4,-0.4) grid (0.8,0.8);

     \draw[step=0.4cm,black,thick] (-1.2,-1.2) grid (1.6,1.6);

    % Optionally, draw the borders of the grid
    \draw[thick] (-1.2,-1.2) rectangle (1.6,1.6);
    
      % Draw the middle point
    \fill[red] (0.2,0.2) circle (1pt);
\end{tikzpicture}
\caption{The grid construction $\bar{V}_i$ around the red point $x_i\in \kapprox$.}
\label{fig:grid}
    \end{minipage}\hfill
    \begin{minipage}{0.49\textwidth}
        \centering
        \begin{tikzpicture}[scale=0.6]
    \draw[thick] (5,5) rectangle (7,7);
    \node[right] at (7,6.8) {$\square_1$};
    \draw[thick] (11.5,1.5) rectangle (13,3);
    \node[right] at (13,2.8) {$\square_2$};
    
    \fill[black] (10,2) circle (4pt);
    \node[above] at (10.2,2.1) {$x_i$};
    \fill[black] (5.5,4) circle (4pt);
    \node[above] at (6.1,4) {$x_{i+1}$};
    \fill[black] (12.5,4) circle (4pt);
    \node[above] at (12.8,4) {$x_{i+2}$};
    \fill[black] (9.5,6) circle (4pt);
    \node[above] at (9.8,6) {$x_{i+3}$};

    \draw[red, dashed, thick] (10,2) -- (7,5);
    \draw[red, dashed, thick] (5.5,4) -- (5.5,5);
    \draw[red, dashed, thick] (5,5) -- (7,7);

    \draw[blue, dashed, thick] (10,2) -- (11.5,2);
     \draw[blue, dashed, thick] (12.5,4) -- (12.5,3);
     \draw[blue, dashed, thick] (11.5,1.5) -- (13,3);
\end{tikzpicture}
\caption{Let $\square_1, \square_2\in \bar{V}_i$. It holds that $\dist(x_i,\square_1)>\dist(x_{i+1},\square_1)+\diameter(\square_1)$ so $\square_1$ is not processed by our algorithm. $x_{i+2}$ is the closest center to $\square_2$, i.e., $\dist(\kapprox,\square_2)=\dist(x_{i+2},\square_2)$ and it holds $\dist(x_i,\square_2)<\dist(x_{i+2},\square_2)+\diameter(\square_2)$, so $\square_2$ is processed by our algorithm. The red (blue) dashed segments represent the distances of $x_i$ to $\square_1$ ($\square_2$), $x_{i+1}$ ($x_{i+2}$) to $\square_1$ ($\square_2$), and the diameter of $\square_1$ ($\square_2$).}
\label{fig:condition}
    \end{minipage}
    %\caption{Combined caption for both figures}
\end{figure}


\begin{comment}
\begin{figure*}[h]
\begin{tikzpicture}[scale=1.2]
    % Draw the grid
    \draw[step=0.1cm,black, thick] (0,0) grid (0.4,0.4);

    \draw[step=0.2cm,black,thick] (-0.4,-0.4) grid (0.8,0.8);

     \draw[step=0.4cm,black,thick] (-1.2,-1.2) grid (1.6,1.6);

    % Optionally, draw the borders of the grid
    \draw[thick] (-1.2,-1.2) rectangle (1.6,1.6);
    
      % Draw the middle point
    \fill[red] (0.2,0.2) circle (1pt);
\end{tikzpicture}
\caption{}
\label{fig:grid}
\end{figure*}
\end{comment}

==> oldExtensions.tex <==

\section{Extensions}
In this section, we design approximation algorithms for other graph types or considering the $\ell_2^d$ metric instead of the $\ell_\infty^d$.
Before we analyze the practical types of bipartite graphs we study, we show an extension of our algorithm in Theorem~\ref{thm:approx}to the $\ptwo$ problem in a type of graph which is very close to the \pbg.

Let $\G(\V,\U,\E)$ be a bipartite graph such that $\V$ is a set of $n_V$ points in $\Re^d$, $\U$ is a set of $n_U$ points in $\Re^d$ and there exists an edge between a pair $v\in \V$ and $u\in \U$ if and only if $\dist(v,u)\leq \delta_u$, where $\delta_u$ is a positive real number. We note that this bipartite graph is quite similar to the \pbg, with a major difference that every $u\in \U$ uses a local threshold $\delta_u$ to decide whether $u$ is connected with any node $v\in \V$. This is a more general graph than the \pbg, for which $\delta_u=\delta$ for every $u\in \U$. We call the more general graph, the \emph{various-disk bipartite graph}.

Theorem~\ref{thm:approx} can be straightforwardly extended to the $\ptwo$ problem for various-disk bipartite graphs.
In fact, the algorithm from Theorem~\ref{thm:approx} is identical even to various-disk bipartite graphs. The only difference is that for every $u\in \U$, $\rho_u$ is defined as a box of side length $2\delta_u$ instead of side length $2\delta$.
The algorithm is correct because in the $i$-th iteration of the greedy algorithm, all vertices $\Vnodes(S_i^*)$ must lie in $\rho_i=\bigcap_{u\in \Unodes(S_i^*)}\rho_u$, which is defined as a hyper-rectangle in $\Re^d$. Recall from the definition of the range tree that for any hyper-rectangle $\rho$ in $\Re^d$ it is known that there exists a subset of $O(\log^d n_V)$ canonical nodes that contain all points in $\rho\cap \V$.
Hence, following the proof of Lemma~\ref{lem:corr}, there exists an axis-aligned hyper-rectangle $y$ in $\Re^d$ with the smallest volume that contains all vertices in $\Vnodes(S_i^*)$. The rest of the proof follows verbatim.

\begin{corollary}
\label{cor:approxG}
    Given a various-disk bipartite graph $\G(\V,\U,\E)$ in $\ell^d_\infty$, where $d=O(1)$, such that $n_V=|\V|$, $n_U=|\U|$ (and without loss of generality $n_V\leq n_U$), and $|\E|=m$,  there exists an $O(\log(n_U)\cdot\log^{d} (n_V))$-approximation algorithm for the $\ptwo$ problem for any $c\geq 0$, that runs in $O(n_V\cdot n_U\cdot m^2\cdot \log^{d-1} (n_V)\cdot \log(n_U))$ time.
\end{corollary}

\subsection{Intersection bipartite graphs}


\begin{comment}
\subsection{Interval bipartite graphs}
We show that the $\ptwo$ problem on any interval bipartite graph can be mapped to an instance of the  $\ptwo$ problem in a slight modification of a various-disk bipartite graph in $\ell_\infty^2$.

For every $v\in \V$ (resp. $u\in \U$) let $I_v=[I_v^-, I_v^+]$ (resp. $I_u=[I_u^-, I_u^+])$ be its interval in $\Re^1$. Recall that $(v,u)\in \E$ if and only if $I_v\cap I_u\neq \emptyset$. For every $v\in \V$, let $p_v=(I_v^-, I_v^+)$ be a point in $\Re^2$ with coordinates defined by $I_v^-$ and $I_v^+$. For any $(v,u)\in \E$, we have that $I_v$ intersects with $I_u$. There are four different ways that $I_v$ intersects with $I_u$: i) $I_v^-\leq I_u^-\leq I_v^+\leq I_u^+$, ii) $I_u^-\leq I_v^-\leq I_u^+\leq I_v^+$, iii) $I_v^-\leq I_u^-\leq I_u^+\leq I_v^+$, and iv) $I_u^-\leq I_v^-\leq I_v^+\leq I_u^+$. Equivalently, for every $u\in \U$ we define four rectangles in $\Re^2$: $\rho_u^1=[0,I_u^-]\times [0,I_u^+]$, $\rho_u^2=[I_u^-,\infty)\times [I_u^+,\infty)$, $\rho_u^3=[0,I_u^-]\times [I_u^+,\infty)$, and $\rho_u^4=[I_u^-,\infty)\times [0,I_u^+]$. 
By definition, we note that $I_v\cap I_u\neq \emptyset$ if and only if $p_v\in \rho_u^1$ or $p_v\in \rho_u^2$, or $p_v\in \rho_u^3$, or $p_v\in \rho_u^4$. The side lengths of all rectangles among all points nodes $\U$ might have different side lengths so it defines a various-disk bipartite graph in $\ell_\infty^2$ with the only difference that for each $u\in \U$ there are four rectangles $\rho_u^1,\rho_u^2,\rho_u^3, \rho_u^4$ that whose whose disjunction is used to determine whether $(v,u)\in \E$ for $v\in \V$. The algorithm from Theorem~\ref{thm:approx} (and Corollary~\ref{cor:approxG}) can be extended to work for this extended various-disk bipartite graph.

The algorithm is the same as described in Subsection~\ref{subsec:mainalg}. The only difference is the definition (and computation) of $U_x$ for every canonical node $x$. Recall that we had $U_x=\{u\in \U\mid \square_x\subseteq \rho_u\}$. In the current version, we replace it with $U_x=\{u\in \U\mid \square_x\subseteq (\rho_u^1\cup \rho_u^2\cup\rho_u^3\cup\rho_u^4)\}$. All other steps of the algorithm are identical.
The correctness follows from Lemma~\ref{lem:corr}.
Indeed, in the $i$-th iteration of the greedy algorithm there exists one rectangle $\rho_u\in \{\rho_u^1, \rho_u^2,\rho_u^3,\rho_u^4\}$ for every $u\in\Unodes(S_i^*)$ such that $\Vnodes(S_i^*)\subseteq \bigcap_{u\in \Unodes(S_i^*)}\rho_u$. Hence, there exists an axis-aligned hyper-rectangle $y$ in $\Re^d$ that contains all points in $\Vnodes(S_i^*)$. All other steps of the proof follow verbatim.


\begin{theorem}
\label{thm:intGraph}
    Given an interval bipartite graph $\G(\V,\U,\E)$ such that $n_V=|\V|$, $n_U=|\U|$ (and without loss of generality $n_V\leq n_U$), and $|\E|=m$,  there exists an $O(\log(n_U)\cdot\log^{2} (n_V))$-approximation algorithm for the $\ptwo$ problem for any $c\geq 0$, that runs in $O(n_V\cdot n_U\cdot m^2\cdot \log (n_V)\cdot \log(n_U))$ time.
\end{theorem}
\end{comment}


\begin{comment}
\subsection{Permutation bipartite graphs}
We show that the $\ptwo$ problem on any permutation bipartite graph can be mapped to an instance of the $\ptwo$ problem in a various-disk bipartite graph in $\ell_\infty^2$.
Recall that a permutation bipartite graph is a graph that is both a permutation graph and a bipartite graph.
Assume the diagraph of the permutation of $G$ that consists of an ordering $\sigma(\cdot)$ of the nodes in $\nodes(G)$ and a permutation $\hat{\sigma}(\cdot)$  of the nodes $\nodes(G)$.
For each $v\in \V$ (resp. $u\in \U$), let $I_v$ be a segment that connects the point $(\sigma(v),0)\in \Re^2$ with $(\hat{\sigma}(v),1)\in \Re^2$. 
By definition, $(v,u)\in \E$ if and only if $I_v\cap I_u\neq\emptyset$. Furthermore, since $G$ is both permutation and bipartite we assume that for every different pair $v_1,v_2\in \V$, $I_{v_1}\cap I_{v_2}=\emptyset$.

Based on the discussion above, we define the following bipartite graph $\G'(\V',\U',\E')$.
For every $v\in \V$ we define the point $p_v=(\sigma(v),\hat{\sigma}(v))\in \Re^2$ in $\V'$. For every $u\in \U$ we define the point 
$p_u=(\sigma(u), \hat{\sigma}(u))\in \Re^2$ in $\U'$ with $\delta_{p_u}=\frac{\sigma(u)+\hat{\sigma}(u)}{2}$.

$p_u=\min\{\sigma(u),\hat{\sigma}(u)\}+\frac{\sigma(u)+\hat{\sigma}(u)}{2}\in \Re$ in $\U'$ with $\delta_{p_u}=\frac{\sigma(u)+\hat{\sigma}(u)}{2}$. We make the following observation.

\begin{lemma}
For any $v\in \V$ and $u\in \U$,
    $(v,u)\in \E$ if and only if $\dist(p_v,p_u)\leq \delta_{p_u}$.
\end{lemma}
\begin{proof}
    If $(v,u)\in \E$ then $I_v\cap I_u\neq \emptyset$. Recall that the segment $I_u$ connects $(\sigma(u),0)$ with $(\hat{\sigma}(u),1)$. Let $I_u'$ be its projection on the horizontal line $y=0$, i.e., $I_u'=[\min\{\sigma(u),\hat{\sigma(u)}\}, \max\{\sigma(u),\hat{\sigma(u)}\}]$. Since $I_v$ intersects with $I_u$ we have that $\sigma(v)\in I_u'$. Notice that $p_v=\sigma(v)$ and $p_u$ is defined as the middle point of $I_v'$. Hence, $\sigma(v)\in I_u' \Leftrightarrow \dist(p_v,p_u)\leq \delta_{p_u}$.

    
    \end{proof}

Hence, the new graph $\G'$ is a various-disk bipartite graph in $\ell_\infty^1$. We conclude with the next theorem.

\begin{theorem}
\label{thm:permGraph}
    Given a permutation bipartite graph $\G(\V,\U,\E)$ such that $n_V=|\V|$, $n_U=|\U|$ (and without loss of generality $n_V\leq n_U$), and $|\E|=m$,  there exists an $O(\log(n_U)\cdot\log (n_V))$-approximation algorithm for the $\ptwo$ problem for any $c\geq 0$, that runs in $O(n_V\cdot n_U\cdot m^2\cdot \log(n_U))$ time.
\end{theorem}
\end{comment}



\subsection{$k$-NN bipartite graphs}
We show that the $\ptwo$ problem on any $k$-NN bipartite graph can be mapped straightforwardly to an instance of the $\ptwo$ problem in a various-disk bipartite graph in $\ell_\infty^d$. Indeed, for every $u\in \U$, we define a box $\rho_u$ in $\Re^d$ with side-length $2\dist(u,\textsf{k-NN}(u,V))$, where $\textsf{k-NN}(u,V)$ is the $\ell_\infty$ distance of $u$ with its $k$-nearest neighbor in $V$. We can precompute all these boxes in $O(n_U\cdot n_V)$ time. Then we notice that this is an instance of the $\ptwo$ problem in a various-disk bipartite graph in $\ell_\infty^d$.

\begin{theorem}
\label{thm:kNNGraph}
    Given a $k$-NN bipartite graph $\G(\V,\U,\E)$ in $\ell_\infty^d$, where $d=O(1)$, such that $n_V=|\V|$, $n_U=|\U|$ (and without loss of generality $n_V\leq n_U$), and $|\E|=m$,  there exists an $O(\log(n_U)\cdot\log^d (n_V))$-approximation algorithm for the $\ptwo$ problem for any $c\geq 0$, that runs in $O(n_V\cdot n_U\cdot m^2\cdot\log^{d-1}(n_V) \cdot \log(n_U))$ time.
\end{theorem}


\subsection{Extension to $\ell_2^d$}

==> oldVersion.tex <==
\stavros{-------OLD---------}
Bipartite graphs play an important role in computer science modeling instances of problems in various areas such as social network analysis, job matching, dating platforms, recommendation systems, resource allocation~\cite{wellman1997structural}, etc.
In this paper, we focus on variants of a well-studied problem in bipartite graphs, called the \emph{minimum biclique cover problem} or the \emph{bipartite dimension problem}.
Given a bipartite graph $\G(\V,\U,\E)$, the goal is to find the minimum number of complete bipartite subgraphs (also called \emph{bicliques}) to cover all edges in $\E$. Similar to the minimum biclique cover problem, there exists the minimum biclique partition problem, where the goal is to find the minimum number of bicliques that partition the edges of a bipartite graph. The bipartite dimension problem has many applications in computer science, such as automata and language theory~\cite{gruber2007inapproximability}, computer security~\cite{ene2008fast}, bioinformatics~\cite{nau1978mathematical}, graph drawing~\cite{eppstein2007confluent}, and data mining \cite{edge-RMP-hardness, role-mining-survey}. Another interesting application of the bipartite dimension problem comes from linear algebra. Given a Boolean matrix $(M)_{n_1\times n_2}$, the Boolean rank of $M$ denoted by $k$ is the smallest number such as there exist two tables $(A)_{n_1\times k}$ and $(B)_{k\times n_2}$ such that $M=AB$. It is known that computing the Boolean rank of a matrix is equivalent to computing the bipartite dimension of a bipartite graph~\cite{gregory1991biclique}.

Multiple variations of the bipartite dimension problem have been studied in the literature, as discussed in Subsection~\ref{sec:rel}. In this paper, we study two variations and show a connection between these problems with data compression problems. The first variation has been studied in the literature and it is called the \emph{Weighted Biclique Cover} problem ($\pone$). The $\pone$ problem was first defined in~\cite{tarjan1975complexity}. The second problem is a new variation that we define, combining the bipartite dimension with the Weighted Biclique Cover problem, having interesting applications in data compression and communication complexity.

We consider the following scenario. In a cloud computing setting, there are multiple computing machines and links that connect the machines in a network. Alice wants to transfer a bipartite graph $\G(\V,\U,\E)$, which is currently stored in machine $A$, to Bob, who has access only to computing machine $B$.
Similarly, instead of considering a bipartite graph, we can consider a Boolean matrix $(M)_{n_1\times n_2}$. Alice might want to transfer $M$ from machine $A$ to machine $B$. As we mentioned for the bipartite dimension problem, the boolean matrix $M$ can be represented as a bipartite graph $\G_M(\V_M,\U_M,\E_M)$ such that for each row in $M$ there exists a node in $\V_M$, for each column of $M$ there is a node in $\U_M$, and for each $h_1\in[n_1], h_2\in [n_2]$ with $M[h_1,h_2]=\mathsf{true}$ there exists an edge between the corresponding $h_1$ node in $\V_M$ and the corresponding $h_2$ node in $\U_M$. In both cases, we assume that Alice has to transfer a bipartite graph $\G(\V,\U,\E)$.

One option is to transfer the entire graph $\G$ from $A$ to $B$; however, in this case, the network needs to transfer $|\V|+|\U|+|\E|$ ``objects'', which can be too expensive. In order to reduce the number of objects transferred in the network, Alice can use the following idea: Transfer only bicliques of $\G$ so that we do not need to transfer explicitly any edges from $\G$. Let $\edgecover=\{\cover_1,\ldots, \cover_r\}$ be a collection of bicliques of $\G$ that cover all edges in $\E$, i.e., $\bigcup_{\cover_i\in\edgecover}\edges(S_i)=\bigcup_{\cover_i\in\edgecover}\Vnodes(\cover_i)\times \Unodes(\cover_i)=\E$, where $\edges(X)$ is the set of edges in the subgraph $X\subseteq G$, $\Vnodes(X)$ is the set of nodes in $\V$ that exist in $X$, and $\Unodes(X)$ is the set of nodes in $\U$ that exist in $X$. Let also $\nodes(X)=\Vnodes(X)\cup \Unodes(X)$ be the set of nodes in the subgraph $X$. If Alice transfers $\edgecover$ from $A$ to $B$, then Bob can retrieve the original bipartite graph exactly (lossless compression). In this case, the number of objects that are transferred from $A$ to $B$ is $\sum_{\cover_i\in\edgecover}|\Vnodes(\cover_i)|+|\Unodes(\cover_i)|=\sum_{\cover_i\in \edgecover}|\nodes(\cover_i)|$. Hence, if we want to minimize the number of objects transferred from $A$ to $B$ the goal is to find the collection of bicliques $\edgecover$ such that i) the implicit edges in $\edgecover$ cover all edges in $\G$, i.e., $\bigcup_{\cover_i\in\edgecover}\Vnodes(\cover_i)\times \Unodes(\cover_i)=\E$ and ii) the number of transferred objects is minimized, i.e., $\sum_{\cover_i\in\edgecover}|\nodes(\cover_i)|$ is minimized. This is exactly the definition of the $\pone$ problem.

We note the difference between the bipartite dimension problem and the $\pone$ problem. In the $\pone$ problem, notice that the number of bicliques does not matter. Instead, only the total size of the bicliques matters. Indeed, in the lossless bipartite graph compression application defined above, we only care about the total number of objects transferred from machine $A$ to machine $B$. However, in real systems, each biclique transferred from $A$ to $B$ might need to transfer additional information so that Bob can reconstruct the original graph $\G$. For example, Alice needs to add a header in front of each new biclique $\cover_i$ transferred from $A$ to $B$ so that Bob knows the nodes assigned to each biclique. More generally, for transferring each biclique $\cover_i$ through the network, some additional transferring cost needs to be paid. Another example is that if each biclique is transferred via a separate package in the network, then each package needs to store additional information that is also transferred from $A$ to $B$. Let $c$ be the additional transferring cost that needs to be paid for every biclique transferred in the network.
This is the motivation of the new variant defined in this paper, called \emph{Generalized Weighted Biclique Cover} ($\ptwo$) problem. In this case, in order to minimize the number of objects transferred from $A$ to $B$ the goal is to find the collection of bicliques $\edgecover$ such that i) the implicit edges in $\edgecover$ cover all edges in $\G$, i.e., $\bigcup_{\cover_i\in\edgecover}\Vnodes(\cover_i)\times \Unodes(\cover_i)=\E$ and ii) the transferring cost is minimized, i.e., $c\cdot |\edgecover|+\sum_{\cover_i\in\edgecover}|\nodes(\cover_i)|$ is minimized. 
In most realistic scenarios, the additional transfer cost $c$ is small. 
For instance, when transmitting packets over a network, the header overhead is bounded by a constant independent of the data payload size (e.g., the IPv4 or TCP header is 20 bytes). 
In contrast, if $c$ is very large, say $c \geq (|\V|+|\U|)^6$, then the term $c \cdot r$ always dominates the cost $\sigma(\edgecover)$ in the $\ptwo$ problem. 
In this case, the problem effectively reduces to minimizing the number of bicliques in the cover, i.e., the bipartite dimension problem.
%, which is known to be NP-complete.



It is known that the decision version of the bipartite dimension problem is NP-complete~\cite{gottlieb2005efficient, orlin1977contentment}. Moreover, the $\pone$ decision problem is shown to be NP-complete in at least two different works \cite{Drawing-Hardness, edge-RMP-hardness}, from different fields by different reductions. These results directly imply the NP-completeness of $\ptwo$, when $c = 0$, as the two problems become equivalent. In this work, we show that $\ptwo$ is NP-complete for every fixed integer parameter $c > 0$.


Interestingly, although the $\pone$ and $\ptwo$ problems have important applications in data compression and cloud computing, to the best of our knowledge, no approximation algorithms with theoretical guarantees are known. 
We build on the observation that many graphs arising in practice are naturally \emph{disk graphs}~\cite{atminas2018forbidden, lahn2021faster,lokshtanov2024bipartizing} (also referred to as \emph{proximity graphs}~\cite{agarwal2024reporting} or \emph{intersection graphs}~\cite{har2025approximating, har2022approximation, jana2023maximum}) or can be well approximated as such. 
In these graphs, nodes are embedded as points in a low-dimensional geometric space, and edges connect pairs of nodes that are sufficiently close. 
For example, social networks and co-authorship graphs can often be embedded, with small error, into the space of user profiles with low intrinsic dimension~\cite{verbeek2014metric, yang2012defining}. 
More generally, for many networks across diverse domains (e.g., social, transportation, Internet), suitable embeddings exist that approximately preserve structural properties and shortest paths of the original graphs~\cite{verbeek2014metric, zhao2010orion, zhao2011efficient}. 
This key observation allows us to exploit the structure of disk graphs to design approximation algorithms for $\pone$ and $\ptwo$, thereby overcoming the hardness of these problems on arbitrary graphs.
Finally, various optimization problems considered bipartite structures in disc graphs~\cite{atminas2018forbidden, jana2023maximum, lahn2021faster, lokshtanov2024bipartizing}. For example, Lahn et al.~\cite{lahn2021faster} studied the maximum cardinality bipartite matching problem on $\delta$-disc bipartite graphs.

%Finally, many optimization problems consider disk bipartite 



%Interestingly, the complexity of the $\pone$ and $\ptwo$ problem have not been studied before. In fact, in~\cite{tarjan1975complexity}, where $\pone$ is first defined, the authors left the complexity of the problem as an open problem.
%All papers that have studied $\pone$~\cite{chung1983decomposition, davoodi2016edge, tarjan1975complexity, tuza1984covering} focused on computing upper and lower bounds on the cost of the optimum solution (sum of sizes of bicliques in the optimum solutions). We solve this long-standing problem by proving that $\pone$ is NP-complete. Furthermore, we are the first that study the hardness of $\ptwo$.


\subsection{Our contributions}

\stavros{-----OLD-------}
While the $\pone$ problem is known to be NP-complete, to the best of our knowledge, the existing proofs~\cite{Drawing-Hardness, edge-RMP-hardness} cannot be trivially extended to show the NP-completeness of $\ptwo$, for $c > 0$. To this end, we first show a new proof of NP-completeness for $\pone$ using a reduction from the 3SAT problem. Then we extend the ideas to show that $\ptwo$ is also NP-complete for any fixed integer parameter $c \geq 0$. 


No approximation algorithms have been studied for the $\pone$ problem (and its generalization $\ptwo$) on general graphs or even on restricted classes. 
Our work provides the first approximation algorithms for these problems in a non-trivial graph class, namely disk graphs under the $\ell^d_\infty$ metric. 

We begin by showing that $\ptwo$ can be reduced to a weighted set cover instance with exponentially many sets. 
Exploiting the geometric structure of a $\delta$-disk bipartite graph $\G(\V,\U,\E)$ in $\ell^d_\infty$, we design an approximation of the classical greedy set cover algorithm that avoids constructing all sets explicitly. 
In particular, in each iteration we compute a set whose cost ratio (weight divided by the number of newly covered elements) is at most $O(\log^d \min\{|\V|,|\U|\})$ times larger than that of the optimal set.
Letting $n_V = |V|$, $n_U = |U|$ (without loss of generality assume that $n_V \leq n_U$), and $m=|\E|$, we obtain an $O(\log(n_U)\cdot \log^d(n_V))$-approximation algorithm for the $\ptwo$ problem (for any real parameter $c \geq 0$) that runs in 
$O\left(n_V \cdot n_U \cdot m^2 \cdot \log^{d-1}(n_V)\cdot \log(n_U)\right)$
time. 
Since the algorithm applies to every $c \geq 0$, it also yields a valid approximation algorithm for the $\pone$ problem.


\subsection{Related work}
There is a lot of related work on computing the bipartite dimension of a bipartite graph. First, Orlin~\cite{orlin1977contentment} showed that the bipartite dimension problem is NP-complete. The problem remains NP-hard even if the input bipartite graph has bipartite dimension $O(\log n)$, where $n$ is the size of the given instance~\cite{gottlieb2005efficient}.

Since the bipartite dimension problem is NP-complete, the existence of approximation algorithms has also been studied. Simon~\cite{simon1990approximate} showed that the bipartite dimension problem is NP-hard to approximate within a factor $n^{1-\eps}$, for any fixed $\eps>0$, where $n$ is the number of nodes. Gruber and Holzer~\cite{gruber2007inapproximability} used the construction from~\cite{simon1990approximate} to show that the problem is $n^{1/3-\eps}$ and $m^{1/5-\eps}$ hard to approximate, where $n$ is the number of nodes and $m$ is the number of edges in the input bipartite graph.
Chalermsook et al.~\cite{chalermsook2014nearly} showed that the minimum biclique edge cover (bipartite dimension problem) and the minimum biclique edge partition problem on bipartite graphs are as hard to approximate as the graph coloring problem. Combining this result with the hardness results for graph coloring~\cite{feige1998zero, khot2006better, zuckerman2006linear}, it implies that these problems do not admit $n^{1-\eps}$ and $m^{1/2-\eps}$ approximation algorithm unless P=NP.

In contrast, the bipartite dimension problem is fixed-parameter tractable.
It is known~\cite{fleischner2009covering, nor2012mod} that the problem can be solved in time $O(f(k)\cdot\poly(n))$ provided that a biclique cover of size $k$ exists, where $f(k)$ is a real function that depends on $k$. Later, Chandran et al.~\cite{chandran2017parameterized} improved the exact running time complexity.


Interestingly, the bipartite dimension problem can be solved exactly in polynomial time in several graph classes, such as domino-free graphs, C4-free graphs, bipartite permutation graphs, bipartite distance-hereditary graphs, and bipartite convex graphs~\cite{amilhastre1998complexity, lubiw1991weighted, muller1996edge}.
Fast heuristics~\cite{ene2008fast} have also been studied for the bipartite dimension problem, however, these methods do not give a theoretical guarantee.

Different versions of the minimum biclique edge cover have been studied~\cite{orlin1977contentment}, like finding the minimum number of bicliques that cover all vertices of a bipartite graph~\cite{ivanescu1967boolean}.


The $\pone$ problem was first defined in~\cite{tarjan1975complexity}. It was the first time that a variant of the biclique edge cover considered the size of the bicliques instead of the number of them. Later, more papers~\cite{chung1983decomposition, davoodi2016edge, tuza1984covering} studied the $\pone$ problem, also called the Weighted Biclique Cover problem.
However, they all give upper and lower bounds on the cost of the optimum solution of the $\pone$ problem, and they do not discuss its complexity. The complexity of $\pone$ was first discussed in~\cite{Drawing-Hardness}, and the problem is shown to be NP-complete in~\cite{Drawing-Hardness, edge-RMP-hardness}. For a nice survey discussing the importance of the $\pone$ problem and its variants in data mining, see~\cite{role-mining-survey}. To the best of our knowledge, there are no approximation algorithms or inapproximability results known for $\pone$ or $\ptwo$. Only heuristics and greedy algorithms without specific theoretical guarantees have been considered in the literature~\cite{role-mining-survey, newbery1989edge, edge-RMP-hardness}.
While there are some results for the weighted biclique edge partition problem~\cite{chavan2025clique, FEDERcompress}, to the best of our knowledge these results cannot be extended to the $\pone$ (or $\ptwo$) problem.

We present the first approximation algorithms for both the $\pone$ and $\ptwo$ problems on $\delta$-disk bipartite graphs. 
A variety of problems have been studied on $\delta$-disk graphs (not necessarily bipartite), including the densest subgraph problem~\cite{har2025approximating}, the maximum clique problem~\cite{clark1990unit}, and others~\cite{agarwal2014near, chekuri2020fast}. 
Recently, Lahn et al.~\cite{lahn2021faster} designed an efficient algorithm for the maximum cardinality bipartite matching problem on $\delta$-disk bipartite graphs. 
The objectives of these problems, however, are fundamentally different from those considered in our work.


Finally, a related problem called the maximum edge biclique problem has been studied in the literature. In the maximum edge biclique problem, the input is a bipartite graph and the goal is to find the biclique with the largest number of edges, i.e., find the biclique $S$ in the input bipartite graph $\G$ such that $|\edges(S)|$ is maximized. First, the weighted version of the maximum edge biclique problem (where the goal is to find the biclique with the minimum sum of edge weights) was proven to be NP-complete~\cite{dawande1996biclique}; later, the unweighted version was also shown to be NP-complete~\cite{peeters2003maximum}. Inapproximability results for the maximum edge biclique problems are also known~\cite{ambuhl2011inapproximability, feige2002relations}.

==> proofs.tex <==
\section{Hardness of $\pone$}
While the hardness of the $\pone$ problem is known, we show a new proof to set the stage for our main hardness results described in Section~\ref{sec:gwbc-hard}.
We start by showing that $\pone$ is NP-complete by a polynomial reduction from the $3SAT$ problem, which is well-known to be NP-complete.



\input{torus}

\begin{definition}
    (3SAT) A set of $n$ clauses $C = \{C_1, \dots, C_n \}$, over $s$ variables $b_1, \dots, b_s$ is given. Each clause $S_i$ consists of three literals $l_{i,1}, l_{i,2}, l_{i, 3}$ where a literal $l_{i,j}$ is either a variable or its negation. The problem is to determine whether there exists a truth assignment to the variables such that each clause has at least one true variable. 
\end{definition}

The main idea of the reduction is the following. Given an instance of the $3SAT$ problem, we build a bipartite graph $H$, such that by solving $\pone$ on $H$, we can decide the satisfiability of the given $3SAT$ instance. To build such a graph $H$, we use the elegant idea of \cite{Holyertorus} that is tiling the torus with graphs. However, instead of tiling with complete graphs as in \cite{Holyertorus}, we tile the torus by rectangles ($K_{2,2}$). We note that the terms rectangles, cycles of length 4, and complete bipartite graphs having $2$ nodes on each part are used interchangeably and denoted by $K_{2, 2}$. We then build $H$ by using copies of these tiled toruses as the building blocks, similar to \cite{FEDERcompress}. Then we show that the minimum cost of $\pone$ on $H$ is achieved when we partition its edges to copies of $K_{2,2}$, if possible (note the difference between partitioning and covering). This means that if it is possible to partition the edges of $H$ into copies of the $K_{2,2}$ graph, the algorithm that solves $\pone$ on $H$ will do that.
%Although it is known that partitioning the edges of such a graph $H$ into copies of $K_{2,2}$ graph is $NP-complete$ as shown in \cite{}, we need to redo some analysis and modify the graphs to later be able to move from the NP-completeness of $\pone$ to $\ptwo$. 

Let $B_p$ be the graph corresponding to the embedding of a $p \times p$ grid on the 2-dimensional torus (the toroidal $p \times p$ grid), for a sufficiently large even number $p$. An illustration is shown in Figure \ref{fig:figure1}. One can think of $B_p$ as the tiling of a torus by rectangular tiles, while $p$ determines the number of tiles used in each direction. The main property of $B_p$ is that its edges can be partitioned to $K_{2,2}$ graphs in exactly two ways, and this property can be used to build switches for simulating a 3SAT instance.

\begin{lemma} \label{lem:two}
    The edges of the graph $B_p$ can be partitioned into copies of $K_{2,2}$ in exactly two different ways for any even $p \geq 2$. Two partitions are considered different if there exist two edges of $B_p$ like $e_1$ and $e_2$, such that in one partition they belong to the same $K_{2,2}$, and in the other partition they do not. 
\end{lemma}
\begin{proof}
    Consider an arbitrary rectangle in $B_p$ called $t$. There are two ways to partition the edges of $t$, i) all the edges of $t$ belong to the same $K_{2,2}$ in the partition, or ii) the edges of $t$ are partitioned by $4$ different copies of $K_{2, 2}$. In both cases, the rest of the graph is partitioned uniquely when $p$ is even. So, there are exactly two different partitions for $B_p$.
\end{proof}

Following the notation of \cite{Holyertorus}, we have the following definitions:

\begin{definition}
    According to Lemma \ref{lem:two}, we know that the edges of $B_p$ can be partitioned into copies of $K_{2,2}$, in exactly two ways. We call one partition the $T$-partition and the other one the $F$-partition.
\end{definition}

\begin{definition}
    Two rectangles are called neighbors if they share an edge.
\end{definition}

\begin{definition}
    A patch is an induced subgraph of a rectangle in $B_p$ and all of its neighboring rectangles (see Figure~\ref{fig:figure2}).
\end{definition}

\begin{definition}
    A patch is a $T$-patch if its centering rectangle belongs to the $T$-partition and an $F$-patch if it belongs to the $F$-partition.
\end{definition}
The distance between two vertices $v, u$ in a graph $G$ is defined as the length of the shortest path from $v$ to $u$. The distance between two patches $P_1, P_2$ in $G$ is the smallest distance between any pair of vertices $(p_1,p_2)\in P_1\times P_2$.
\begin{definition}
    Two different patches are far if the distance between them is at least $50$.
\end{definition}
    We note that the number $50$ in the above definition is just an arbitrary number that is sufficiently large. 
    Given a pair of graphs $G_1$ and $G_2$, we use the term $G_1 \subset G_2$ to denote that $G_1$ is a subgraph of $G_2$. Next, we define the \textit{join} operation between a pair of graphs on a pair of patch subgraphs.
    Let $Q_1$ and $Q_2$ be arbitrary graphs and $P_1$ and $P_2$ be a pair of patches, such that $P_1 \subset Q_1$ and $P_2 \subset Q_2$.
    %We are given two graphs $Q_1$ and $Q_2$ and two patches $P_1\subset Q_1$ and $P_2\subset Q_2$. 
    By the definition of patches, we know that $P_1$ and $P_2$ are isomorphic. Let $\mathsf{Border}(P_1)=\{v_1, v_2, v_3, v_4, v_5, v_6, v_7, v_8\}$ be the vertices in $\nodes(P_1)$ that are connected with vertices in $\nodes(Q_1)\setminus\nodes(P_1)$, i.e., these are all the vertices of a patch except of the vertices in its central rectangle. Similarly, we define $\mathsf{Border}(P_2)=\{u_1,u_2, u_3, u_4, u_5, u_6, u_7, u_8\}$ for $P_2$.
    For a vertex $v_i$ for $i\in\{1,\ldots, 8\}$ let $v_i^{(1)}$ and $v_i^{(2)}$ be the two vertices in $\nodes(Q_1)\setminus \nodes(P_1)$ that are connected with $v_i$. Similarly, for each vertex $u_i$, we define  $u_i^{(1)}$ and $u_i^{(2)}$.
    Let $Q_1'=Q_1\setminus P_1$ and $Q_2'=Q_2\setminus P_2$, i.e., we remove the patches along with all incident edges from their graphs $Q_1$ and $Q_2$.
      We build a new graph $Q_3'=Q_1'\cup Q_2'$. Let $P_{1,2}$ be a patch isomorphic to $P_1$ and $P_2$ with $\mathsf{Border}(P_{1,2})=\{y_1,y_2, y_3, y_4, y_5, y_6, y_7, y_8\}$. We define the \emph{join} operation of $Q_1$ and $Q_2$ on the patches $P_1$ and $P_2$ as the graph $Q_{1,2}$ with vertices $\nodes({Q_1'})\cup\nodes({Q_2'})\cup\nodes({P_{1,2}})$ and edges $$\edges(Q_1')\cup\edges(Q_2')\cup\edges(P_{1,2})\bigcup_{y_i\in \mathsf{Border}(P_{1,2})}\left(\left(y_i,v_i^{(1)}\right)\cup \left(y_i,v_i^{(2)}\right)\cup \left(y_i,u_i^{(1)}\right)\cup \left(y_i,u_i^{(2)}\right)\right).$$


    \begin{comment}
    Let $N(P_1)=\{v\in Q_1\setminus P_1, \exists p\in \nodes{P_1}: (v,p)\in \edges(Q_1)\}$ and 
    $N(P_2)=\{u\in Q_2\setminus P_2, \exists p\in \nodes{P_2}: (u,p)\in \edges(Q_2)\}$
    be the neighboring vertices of $P_1$ in $Q_1$ and the neighboring vertices from $P$ in $Q_2$, respectively.
    Let $Q_1'=Q_1\setminus P_1$ and $Q_2'=Q_2\setminus P_2$, i.e., we remove the patches along with all incident edges from their graphs $Q_1, Q_2$.
    We define the \emph{join} operation of $Q_1$ and $Q_2$ on the patches $P_1$ and $P_2$ as follows. We build a new graph $Q_3'=Q_1'\cup Q_2'$.


\begin{definition}
    Given a graph $G$ and two vertices $v_1, v_2 \in V(G)$, the following operation is called \textit{joining} $v_1$ and $v_2$: We add a new vertex $v_3$ and add an edge between $v_3$ and all the nodes in $N(v_1) \cup N(v_2)$. Then we remove $v_1$ and $v_2$ and all their neighboring edges from $G$. We call the newly added vertex $v_3$ the \textit{merge point}.
    Also, given two ordered sets of vertices $S = \{ s_1, \dots, s_r \}$ and $T = \{ t_1, \dots, t_r \}$, such that $S, T \subseteq V(G)$ and $|S| = |T|$, joining $S$ and $T$ means joining the nodes $s_i$ and $t_i$ for all $i \in [r]$.  We call the set of all the newly added vertices the \textit{merge points}.
\end{definition}

\begin{definition}
    Given two graphs $Q_1$ and $Q_2$ and two patches $P_1 \subset V(Q_1)$ and $P_2 \subset V(Q_2)$\footnote{Here we assume that $Q_1$ and $Q_2$ have a patch as their subgraphs.}, \textit{joining} $Q_1$ and $Q_2$ on the patches $P_1$ and $P_2$, means the following operation: We build a new graph $Q_3 = Q_1 \cup Q_2$, and order the two patches $P_1$ and $P_2$ in the same way to get two ordered sets of vertices $P'_1, P'_2 \subset Q_3$. At last, we join the two ordered sets $P'_1$ and $P'_2$ in $Q_3$ and return $Q_3$ as the result. 
    \end{definition}
\end{comment}
 Given three graphs $Q_1, Q_2, Q_3$ and three patches $P_1\subset Q_1, P_2 \subset Q_2, P_3 \subset Q_3$ from them, joining them means first joining $Q_1$ and $Q_2$ on $P_1$ and $P_2$ and then joining the resulting graph $Q_{1,2}$ with $Q_3$ on the patches $P_{1,2}$ and $P_3$.

\paragraph{Construction of polynomial time reduction}
The construction is similar to the construction in~\cite{Holyertorus}.
Suppose that an instance of the 3SAT problem $C = \{ C_1, \dots, C_{n}$\} over the variables $b_1, \dots, b_s$ where $C_i$ consists of $l_{i,1}, l_{i,2}, l_{i,3}$ is given. We choose a sufficiently large $p$, say $p = 500n$. Then, we build the graph $H$ using copies of $B_p$ as follows. For each variable $b_i$, we use a copy of $B_p$, called $F_i$. Also, for each clause $C_i$, we take three copies of $B_p$, called $C_{i, 1}, C_{i, 2}, C_{i, 3}$. Now we stick these copies of $B_p$ together as follows. For each $C_i$, find one $F$-patch from each of the $C_{i, 1}, C_{i, 2}$, and $C_{i, 3}$. Then, join together all these three copies on the selected $F$-patches. Let $P$ be the new patch that $C_{i, 1}, C_{i, 2}$, and $C_{i, 3}$ are connected through. We remove the edges of the central rectangle of patch $P$.
Then, if the variable $l_{i,j}$ is $b_h$, find an $F$-patch of $C_{i, j}$ and an $F$-patch of $F_h$ and join them on the corresponding $F$-patch. If $l_{i,j}$, is the negation of $b_h$, do the same operation but by joining an $F$-patch of $C_{i,j}$  with a $T$-patch of $F_h$. At each step, on the same copy of $B_p$, we choose different $F$-patches such that they are far from each other to ensure that they do not share an edge. Let $H$ be the final graph after doing all the joins. The following result follows from~\cite{FEDERcompress}.
\begin{lemma}\label{theorem:parsat}
 The edges of the graph $H$, as constructed above, can be partitioned into copies of $K_{2,2}$, if and only if the given instance of the 3SAT problem $C$, is satisfiable.
\end{lemma}

%Having the above lemma, we can deduce that for a graph such as $H$, deciding whether it can be partitioned to $K_{2, 2}$, is NP-complete. 

Now we move back to the problem of covering the edges instead of partitioning. We use the nice properties of $H$, to show that $\pone$ is NP-complete. First, observe that by construction every pair of vertices in $H$, have at most $2$ neighbors in common. This property implies that any complete bipartite subgraph of $H$ is either a $K_{2, 2}$ or a $K_{1, t}$ (the $t$-star graph) for some $t$. More importantly, $H$ is a bipartite graph as it does not contain any odd cycles, by its construction.

\begin{theorem} \label{theorem:main1}
    The $\pone$ problem is NP-complete.%More specifically it is NP-complete for a graph $H$ as constructed above. 
\end{theorem}
\begin{proof}
    We first show that $\pone$ is in NP. Let $\edgecover=\{\cover_1,\ldots, \cover_r\}$ be a set of subgraphs returned by an algorithm. First, we check whether $\edgecover$ is a biclique edge covering of $H$. For every $\cover_i\in \edgecover$, we visit each edge $e\in \edges(\cover_i)$. If $e$ is not marked in $H$ we mark it. In the end, after visiting all subgraphs in $\edgecover$, we check whether there exists an unmarked edge in $\edges(H)$. If yes, then we return that $\edgecover$ is not a biclique edge covering of $H$. If no, we check whether $\mu(\edgecover)\leq \tau$. We simply go over all subgraphs in $\edgecover$ and we compute $\mu(\edgecover)=\sum_{\cover_i\in \edgecover}|\nodes(\cover_i)|$. In the end if $\mu(\edgecover)\leq \tau$ we return yes. Otherwise, we return no.

    Given an instance of the 3SAT problem, we construct the graph $H$ as described above. We know that any biclique subgraph of $H$ is either a $t$-star or a $K_{2,2}$.
    %So, the final edge cover of $H$ will only contain one of these two types of bicliques. 
    Now note that by the definition (Definition~\ref{def:wbc}) of the cost function $\mu(\cdot)$ in $\pone$, $K_{2,2}$ has cost $\mu(K_{2,2})=4$ and it covers 4 edges, while a $t$-star $K_{1,t}$ has cost $\mu(K_{1,t})=t+1$ and it covers $t$ edges. Thus, the edges of $H$ can be partitioned to copies of $K_{2, 2}$, if and only if there is a biclique edge cover $\edgecover$ of $H$ such that $\mu(\edgecover)=|\edges(H)|$, so we select $\tau=|\edges(H)|$. According to Lemma~\ref{theorem:parsat}, we know that deciding whether $H$ can be edge partitioned to $K_{2, 2}$ is NP-complete. Therefore, $\pone$ is also NP-complete.
\end{proof}



==> proofs2.tex <==
\section{Hardness of $\ptwo$}\label{sec:gwbc-hard}

\input{bigraph}



It is known that the problem of covering the edges of a bipartite graph using the minimum number of bicliques is NP-complete \cite{orlin1977contentment}. In the previous section, we showed that the problem of minimizing the total size of these bicliques is also NP-complete. However in many applications, both minimizing the number of these bicliques and the total size of them is important, as we highlighted in Section~\ref{sec:intro}. %We can capture this by moving from $\pone$ to $\ptwo$.
Notice that for an instance of the $\ptwo$, if $c = 0$, we have an instance of $\pone$, and if $c$ is equal to a large number, say $c \geq n^6$, where $n$ is the number of the vertices in the input graph, we have an instance of minimizing the number of the bicliques in the cover (the bipartite dimension problem). So, for the two extreme cases of the parameter $c$, we know that the resulting problem is NP-complete. In this section, we show that for any fixed integer value of $c$, the problem of $\ptwo$, is NP-complete. In the proof of Theorem~\ref{theorem:main1}, we used the fact that for the minimum cost edge cover of $H$, it is always preferable to use $K_{2, 2}$ bicliques instead of the $t$-stars. However, if we consider $\ptwo$ with $H$ as its input, it may be better to use one large $t$-star subgraph to pay the cost $c$ once, instead of using multiple $K_{2, 2}$ and paying $c$ multiple times. To address this issue, we first build the graph $H$ as described in the previous section, and then use $H$ as the building block of an even bigger graph, denoted by $H'$. Then, we show that solving $\ptwo$ on $H'$ is NP-complete. 
    
\paragraph{Construction of polynomial time reduction}

We show that $\ptwo$ is NP-complete, by a reduction from the 3SAT problem. Given an instance $C$ of the 3SAT, we build the graph $H$ as described in the previous section. During the process of constructing $H$, we joined at most $3$ different copies of $B_p$ on the same patch, and thus the maximum degree of a vertex in $H$ is $8$. We also know that $H$ is a bipartite graph, by its construction. We make $4c$ copies of $H$. Let $H_i$ denote the $i$'th copy of $H$ and $V_i = \Vnodes(H_i)=\{v_{i,1}, \dots, v_{i, n_1} \}$ and $U_i =\Unodes(H_i)= \{u_{i,1}, \dots, u_{i, n_2} \}$ denote the set of vertices in each part. In this newly made graph of $4c$ copies of $H$, if a node $v_{i,j_1}$ has an edge to $u_{i, j_2}$, we also connect $v_{i,j_1}$ to all the nodes in $\bigcup^{4c}_{k = 1}u_{k,j_2}$ and name the resulting graph $H'$ as shown in Figure \ref{fig:bipartite_graphs}. Our goal is to show that given the answer of $\ptwo$ over $H'$, we can decide whether $C$ is satisfiable and hence $\ptwo$ is NP-complete. 

    \begin{lemma} \label{lem:types}
        Any complete bipartite subgraph of $H'$ denoted by $X$, has one of the following structures:
        \begin{itemize}
            \item (Type-1): For all $i \in [4c]$, the subgraph $X$ has at most $2$ vertices from $V_i$ and at most $2$ vertices from $U_i$.
            \item (Type-2): There exists an $i \in [4c]$, such that $X$ has more than 2 vertices from $V_i$. In this case, for every $j \in [4c]$, the subgraph $X$ has at most one vertex from $U_j$.
            \item (Type-3): There exists an $i \in [4c]$, such that $X$ has more than 2 vertices from $U_i$. In this case, for every $j \in [4c]$, the subgraph $X$ has at most one vertex from $V_j$.
        \end{itemize}
    \end{lemma}
    \begin{proof}
        Assume that $X$ is not of the first type. Since the Type-2 and Type-3 structures are equivalent, without loss of generality we assume that $X$ has more than two vertices from $V_i$, for an index $i$; choose three arbitrary vertices in $V_i$ that are in $X$ denoted by $x_{i_1}, x_{i_2}, x_{i_3}$. We prove by contradiction that $X$ is of the second type. Assume there exists a $j$, such that $X$ has more than one vertex from $U_j$; choose two of them denoted by $y_{j_1}$ and $y_{j_2}$. Since $X$ is a complete bipartite graph, both $y_{j_1}$ and $y_{j_2}$ have an edge to $x_{i_1}, x_{i_2}$, and $ x_{i_3}$.
        By the construction of $H'$, we know that $U_j$ is a copy of $U_i$, so there exist two vertices in $U_i$ (the corresponding copies of $y_{j_1}$ and $y_{j_2}$) that both have an edge to all three $x_{i_1}, x_{i_2}$, and $ x_{i_2}$. By the construction of $H'$, we know that the induced subgraph over $U_i$ and $V_i$ in $H'$, is a copy of $H$ and any two vertices in $H$ have at most two common neighbors, so, this is a contradiction.
    \end{proof}

    For each complete bipartite subgraph $X\subset H'$, we define the \emph{benefit rate} function $f(X)$, as follows:

    \begin{definition}
        (Benefit rate function): For every complete bipartite subgraph $X\subset H'$, the \textit{benefit rate} of $X$ is defines as $f(X) = \frac{|\edges(X)|}{|\Vnodes(X)| + |\Unodes(X)| + c}$.
    \end{definition}
    
    Intuitively, $f(X)$ shows the cost of covering each edge if we use the biclique $X$ in the final cover. 

    \begin{lemma} \label{lem:benef}
    Let $Y$ and $Y'$ be two complete bipartite graphs. If $|\Vnodes(Y)| \geq |\Vnodes(Y')|$ and $|\Unodes(Y)| \geq |\Unodes(Y')|$, then $f(Y) \geq f(Y')$ with equality happening only when $|\Vnodes(Y)| = |\Vnodes(Y')|$ and $|\Unodes(Y)| = |\Unodes(Y')|$.
    \end{lemma}
    \begin{proof}
        We know that $|\Vnodes(Y)| = |\Vnodes(Y')| + a_1$ and $|\Unodes(Y)| = |\Unodes(Y')| + a_2$ where $a_1$ and $a_2$ are non-negative integers. We have $f(Y') = \frac{|\Vnodes(Y')|\cdot|\Unodes(Y')|}{|\Vnodes(Y')| + |\Unodes(Y')| + c}$ and $F(Y) = \frac{(|\Vnodes(Y')| + a_1)(|\Unodes(Y')| + a_2)}{|\Vnodes(Y')| + |\Unodes(Y')| + a_1 + a_2 + c}$. It is straightforward to check that $\frac{(|\Vnodes(Y')| + a_1)(|\Unodes(Y')| + a_2)}{|\Vnodes(Y')| + |\Unodes(Y')| + a_1 + a_2 + c} \geq \frac{|\Vnodes(Y')|\cdot|\Unodes(Y')|}{|\Vnodes(Y')| + |\Unodes(Y')| + c}$, with equality happening only when $a_1 = a_2 = 0$.
    \end{proof}

   \begin{definition}(\emph{Perfect subgraph}): 
        A complete bipartite subgraph of $H'$ is called perfect if it has exactly two nodes from each of the sets $U_i$ and $V_i$ for all $i \in [4c]$.
    \end{definition}

    Assume that $O$ is a complete bipartite subgraph of $H'$, having exactly two nodes from each of the sets $U_i$ and $V_i$ for all $i \in [4c]$. It is easy to check that such a subgraph $O$ exists, but for now, we can just assume its existence. By the definition, we have $$f(O) = \frac{|\edges(O)|}{|\Vnodes(O)|+|\Unodes(O)|+c}=\frac{\sum_{i\in[4c]}4\cdot 4c}{c+\sum_{i\in[4c]}4}=\frac{64c^2}{17c} = \frac{64c}{17}.$$

 

  %  By the definition, we have that for a perfect subgraph, the benefit rate is equal to $\frac{64c}{17}$, like for the subgraph $O$. 
    
    \begin{lemma} \label{lem:perf}
        For any complete bipartite subgraph $X\subset H'$, we have $f(O) \geq f(X)$, with equality happening only when $X$ is perfect.
    \end{lemma}
    \begin{proof}
        We show the correctness by doing a case analysis on the type of $X$ based on the Lemma \ref{lem:types}. If $X$ is of the first type, we have $|\Vnodes(O)| \geq |\Vnodes(X)|$ and $|\Unodes(O)| \geq |\Unodes(X)|$, so according to Lemma \ref{lem:benef}, we have $f(O) \geq f(X)$, with equality happening only when $|\Vnodes(O)| = |\Vnodes(X)|$ and $|\Unodes(O)| = |\Unodes(X)|$, which is the case when $X$ is perfect.

        Now we investigate what happens when $X$ is of the second type. Recall that $H$ has a maximum degree of $8$, and hence for each $i \in [4c]$, every vertex $u \in U_i$ has at most $8$ neighbors in $V_i$. Therefore, $X$ can have at most $8$ vertices from each $V_i$, since it is a complete bipartite graph. So, without loss of generality, we have $|\Vnodes(X)| \leq 8\cdot 4c = 32c$ and $|\Unodes(X)| \leq 4c$ since $X$ is of the second type. Thus, according to the Lemma \ref{lem:benef}, we have $f(X) \leq \frac{(32c)(4c)}{32c + 4c + c} < \frac{64c}{17}$. We know $f(O) = \frac{64c}{17}$, that implies $f(O) > f(X)$.

        With the same analysis as the second case, we can show that if $X$ is of the third type, then $f(O) > f(X)$.
    \end{proof}

     Now, our goal is to prove that if it is possible to partition the edges of $H'$ into perfect subgraphs, the optimal covering of $H'$ will do that. Recall that $\sigma(\cdot)$ is the cost function for $\ptwo$ (see Definition~\ref{def:gwbc}).

     \begin{lemma} \label{lem:opt}
         If $\edgecover = \{\cover_1, \dots, \cover_r \}$ is a biclique edge cover of $H'$, then $\sigma(\edgecover) \geq \frac{17|\edges(H')|}{64c}$, with equality only happening when $S$ partitions the edges of $H'$ into perfect subgraphs.
     \end{lemma}
     \begin{proof}
         For each edge $e \in \edges(H')$, let $\edgecover(e) = \{\cover_i \in \edgecover | e \in \edges(\cover_i) \}$ be the set of bicliques containing the edge $e$, and let $\phi:\edges(H')\rightarrow \Re$ be a real function defined as
         $\phi(e) = \sum_{\cover_i \in \edgecover(e)}\frac{1}{f(\cover_i)}$. Intuitively, by defining $\phi(\cdot)$, we charge each edge by the amount we paid for covering it. 
         Next, we show that $\sigma(\edgecover) = \sum_{e \in \edges(H')}\phi(e)$.
         We have
         \begin{align*}
             \sigma(\edgecover)&=cr+\sum_{\cover_i\in \edgecover}|\nodes(\cover_i)|=\sum_{\cover_i\in \edgecover}(|\Vnodes(\cover_i)|+|\Unodes(\cover_i)|+c)=\sum_{\cover_i\in \edgecover}|\edges(\cover_i)|\frac{|\Vnodes(\cover_i)|+|\Unodes(\cover_i)|+c}{|\edges(\cover_i)|}\\
             &=\sum_{e\in\edges(H')}\hspace{0.8em}\sum_{\cover_i\in \edgecover(e)}\frac{|\Vnodes(\cover_i)|+|\Unodes(\cover_i)|+c}{|\edges(\cover_i)|}=\sum_{e\in\edges(H')}\hspace{0.8em}\sum_{\cover_i\in \edgecover(e)}\frac{1}{f(\cover_i)}=\sum_{e\in\edges(H')}\phi(e).
         \end{align*}
         %It is easy to verify that $\sigma(S) = \sum_{e \in E(H')}\phi(e)$.
         We know that all the edges are contained in at least one $\cover_i$ since $\edgecover$ is an edge cover of $H'$. On the other hand, according to the Lemma \ref{lem:perf}, for all $\cover_i \in \edgecover$, we know that $f(\cover_i) \leq \frac{64c}{17}$, and hence for each $e \in \edges(H)$, we have $\phi(e) \geq \frac{17}{64c}$, where the equality only happens when $e$ is contained in exactly one $\cover_i$, and $\cover_i$ is a perfect subgraph. So, we have,
         \begin{align*}
             \sigma(\edgecover) = \sum_{e \in \edges(H')}\phi(e) \leq  \sum_{e \in \edges(H')}\frac{17}{64c} = \frac{17|\edges(H')|}{64c}.
         \end{align*}
         Where the equality happens only when each $e \in \edges(H')$ is contained in exactly one perfect subgraph. This implies that the equality happens only when $\edgecover$ is an edge partition of $H'$ into perfect subgraphs.
     \end{proof}

     By the following lemma, we show that from an edge partition of $H$ into $K_{2,2}$ graphs an edge partition of $H'$ by perfect subgraphs can be constructed, and vice versa.

     \begin{lemma}\label{lem:part}
         The edges of $H$ can be partitioned into $K_{2, 2}$ subgraphs, if and only if, the edges of $H'$ can be partitioned into perfect subgraphs.
     \end{lemma}
     \begin{proof}
     
         For the first direction, assume that the edges of $H$ can be partitioned into $K_{2, 2}$ subgraphs and let $\edgecover = \{\cover_1, \dots, \cover_r\}$, be this partition. We know that $H'$ is built by the copies of $H$ and the graph induced by each $H_j$ in $H'$, for all $j \in [4c]$ is a copy of $H$. For each $\cover_i \in \edgecover$, we build $\cover'_i$ by adding the corresponding copies of the vertices of $\cover_i$ from each $H_j$, for all $j \in [4c]$. Each $\cover'_i$, is a perfect subgraph of $H'$ since it has exactly two nodes from each $U_j$ and $V_j$, and every node of $\Vnodes(\cover_i')$ has an edge with every node in $\Unodes(\cover_i')$. By the construction of $H'$, it is easy to verify that $\edgecover' = \cup_{\cover_i \in \edgecover} \cover'_i$, is a partition of the edges of $H'$ into perfect subgraphs.

         For the other direction, assume that $\edgecover' = \{\cover'_1, \dots, \cover'_r \}$, is an edge partition of $H'$ into perfect subgraphs. We know that the subgraph $H_1$ in $H'$, is a copy of $H$. For each $\cover'_i \in \edgecover'$, let $\cover_i$ be the graph induced by the corresponding copies of the vertices, i.e., $\{\nodes(\cover'_i) \cap \nodes(H_1)\}$, in $H$. Since $\cover'_i$ is a perfect subgraph, it will have exactly two vertices from both $U_1$ and $V_1$, and hence $\cover_i$ is a $K_{2,2}$ subgraph in $H$. It is easy to verify that $\edgecover = \cup_{\cover'_i \in \edgecover'} \cover_i$, is a partition of the edges of $H$ into $K_{2,2}$ subgraphs.
     \end{proof}

By the following theorem, we show that using the answer of $\ptwo$ on $H'$, we can decide the satisfiability of $C$.
We conclude with the main result in this section.
\begin{theorem}
    The problem of $\ptwo$ is NP-complete, for any fixed integer parameter $c \geq 0$. %\poly(n)$.
\end{theorem}
\begin{proof}
    We first show that $\ptwo$ is in NP. Let $\edgecover=\{\cover_1,\ldots, \cover_r\}$ be a set of subgraphs returned by an algorithm. First, we check whether $\edgecover$ is a biclique edge covering of $H$. For every $\cover_i\in \edgecover$, we visit each edge $e\in \edges(\cover_i)$. If $e$ is not marked in $H$ we mark it. In the end, after visiting all subgraphs in $\edgecover$, we check whether there exists an unmarked edge in $\edges(H)$. If yes, then we return that $\edgecover$ is not a biclique edge covering of $H$. If no, we check whether $\sigma(\edgecover)\leq \tau$. We simply go over all subgraphs in $\edgecover$ and we compute $\sigma(\edgecover)=c\cdot r+\sum_{\cover_i\in \edgecover}|\nodes(\cover_i)|$. In the end if $\sigma(\edgecover)\leq \tau$ we return yes. Otherwise, we return no.


    If $c=0$ then $\ptwo$ is equivalent to $\pone$, so from Theorem~\ref{theorem:main1}, the result follows. Next, we focus on the case where $c > 0$. According to Lemma~\ref{theorem:parsat}, the edges of $H$ can be partitioned into copies of $K_{2,2}$, if and only if $C$ is satisfiable. According to Lemma \ref{lem:part}, the edges of $H$ can be partitioned into copies of $K_{2,2}$ if and only if the edges of $H'$ can be partitioned into perfect subgraphs, and according to Lemma \ref{lem:opt}, the edges of $H'$, can be partitioned into perfect subgraphs if and only if the cost of $\ptwo$ on $H'$ is less than or equal to $\frac{17|\edges(H')|}{64c}$, so we select $\tau=\frac{17|\edges(H')|}{64c}$. Thus, we can decide the satisfiability of $C$ by solving $\ptwo$ over $H'$. The graph $H'$ has $4c$ copies of $H$, and the size of $H$ is polynomially bounded by the size of the 3SAT instance $C$. Since $c$ is a fixed parameter, we can build $H'$ in polynomial time, and the result follows.

    %If $c\geq g^9(n)$, for a polynomial function $g$ with respect to $n$ that we specify later, then notice that for any collection of bicliques $\mathcal{T}=\{T_1,\ldots, T_\ell\}$, of a bipartite graph $G$ with $N$ nodes, where $\ell$ is a positive integer, it holds that $\sum_{T_i\in\mathcal{T}}|\nodes(T_i)|\leq N^3$.
    %It is known from ~\cite{orlin1977contentment} that the bipartite dimension problem is NP-Complete on a graph $\hat{H}$ with $g(n)$ nodes, where $n$ is the number of clauses in the 3SAT instance. In particular, it is NP-Complete to decide whether there exists at most $\rho$ bicliques that cover $\hat{H}$, for a parameter $\rho$. We set $\tau=\rho\cdot g^9(n)+g^3(n)$.
    %If the answer to the bipartite dimension instance is yes for a collection of bicliques $\edgecover=\{\cover_1,\ldots, \cover_\rho\}$, then the instance of $\ptwo$ is also yes because $\sum_{\cover_i\in\edgecover}|\nodes(\cover_i)|\leq g^3(n)$ so $\sigma(\edgecover)\leq \rho\cdot g^9(n) + g^3(n)=\tau$. Similarly, if the instance of $\ptwo$ is yes for a collection of bicliques $\edgecover=\{\cover_1,\ldots, \cover_\ell\}$ then the instance of bipartite dimension problem is also yes. This is because $\sigma(\cover)\leq \rho\cdot g^9(n)+g^3(n)$ and the only way to achieve this cost is by having $\ell\leq\rho$. If $\ell>\rho$ then $\sigma(\cover)$ would be greater than $\rho\cdot g^9(n)+g^3(n)$.

   
    
    %Hence in the cost $\sigma(\cdot)$ selecting only one biclique ($r=1$) always dominates the cost.
    
   % If $c=0$ or $c>n^9$ we have already shown that $\ptwo$ is NP-Complete. 
    
    %Next, we focus on the case where $c=\poly(n)$ and more specifically when $c< g^9(n)$.
    %According to Lemma~\ref{theorem:parsat}, the edges of $H$ can be partitioned into copies of $K_{2,2}$, if and only if $C$ is satisfiable. According to Lemma \ref{lem:part}, the edges of $H$ can be partitioned into perfect subgraphs if and only if the edges of $H'$ can be partitioned into perfect subgraphs, and according to Lemma \ref{lem:opt}, the edges of $H'$, can be partitioned into perfect subgraphs if and only if the cost of $\ptwo$ on $H'$ is equal to $\frac{17|\edges(H')|}{64c}$, so we select $\tau=\frac{17|\edges(H')|}{64c}$. Thus, we can decide the satisfiability of $C$ by solving $\ptwo$ over $H'$. Since $c \in \poly(n)$, and $H'$ has $4c$ copies of $H$, we can build $H'$ in polynomial time and hence we can conclude that $\ptwo$ is NP-complete.

\end{proof}

==> torus.tex <==

\begin{figure}[t]
    \centering
    \begin{minipage}{0.50\textwidth}
        \centering
        \includegraphics[width=0.6\textwidth]{figs/torus_1.png}
        \caption{Overall structure of the embedding of a $p\times p$ grid on the torus. One patch is colored red.}
        \label{fig:figure1}
    \end{minipage}\hfill
    \begin{minipage}{0.44\textwidth}
        \centering
        \includegraphics[width=0.6\textwidth]{figs/torus_2.png}
        \caption{Local structure of a patch.}
        \label{fig:figure2}
    \end{minipage}
    %\caption{Overall caption for both figures}
\end{figure}
